A Reduced Basis Method for the Stochastic Landau-Lifshitz-Gilbert Equation

In this work, we consider the construction of efficient surrogates for the stochastic version of the Landau-Lifshitz-Gilbert (LLG) equation using model order reduction techniques, in particular, the Reduced Basis (RB) method. The Stochastic LLG (SLLG) equation is a widely used phenomenological model for the time evolution of the magnetization field confined to a ferromagnetic body while taking into account the effect of random heat perturbations. This phenomenon is mathematically formulated as a nonlinear parabolic problem, where the stochastic component is represented as a parameter-dependent datum depending on a non-compact and high-dimensional parameter. In an $\textit{offline}$ phase, we use Proper Orthogonal Decomposition (POD) on high-fidelity samples of the unbounded parameter space. To that end, we use the so-called $\textit{tangent plane scheme}$. For the $\textit{online}$ phase of the RB method, we again employ the tangent plane scheme in the RB space. This is possible due to our particular construction that reduces both spaces of the magnetization and of its time derivative. Due to the saddle-point nature of this scheme, a stabilization that appropriately enriches the RB space is required. Numerical experiments show a clear advantage over earlier approaches using sparse grid interpolation. In a complementary approach, we test a sparse grid approximation of the reduced coefficients in a purely data-driven method, exhibiting the weaknesses of earlier sparse grid approaches, but benefiting from increased stability.

==> data_plots/REMOVE/conv_HF_vs_h.tex <==
\begin{figure}
	\center
    % 
	% \includegraphics[width=0.49\textwidth]{data_plots/error_conv_h_HF.png}
	% \includegraphics[width=0.49\linewidth]{data_plots/infsup_conv_h_HF.png}
    % 
    \begin{tikzpicture}
        \begin{loglogaxis}[
            grid=major,
            xlabel={Mesh size $h$},
            legend style={at={(0.97,0.03)}, anchor=south east},
            ymin=1e-2, ymax=4e-1,
            xmin=1e-2, xmax=3e-1,
            width=0.53\linewidth
            ]
            \addplot[mark=*, mark size=1.5pt, blue] table[col sep=comma, x index={0}, y index={2}
            ]{data_plots/1d/conv_test_HF_vs_h.csv};
            \addlegendentry{HF}
            % 
            \addplot[black, thick, domain=2e-2:2e-1, samples=100] {1.2*x};
            \addlegendentry{$h$}
        \end{loglogaxis}
    \end{tikzpicture}
    \begin{tikzpicture}
        \begin{loglogaxis}[
            grid=major,
            xlabel={Mesh size $h$},
            legend style={at={(0.97,0.03)}, anchor=south east},
            ymin=3e-3, ymax=1e-1, 
            xmin=1e-2, xmax=3e-1,
            width=0.53\linewidth
            ]  
            \addplot[mark=*, mark size=1.5pt, blue] table[col sep=comma, x index={0}, y index={3}
            ]{data_plots/1d/conv_test_HF_vs_h.csv};
            \addlegendentry{HF}
            % 
            \addplot[black, thick, domain=2e-2:2e-1, samples=100] {0.2*x};
            \addlegendentry{$h$}
        \end{loglogaxis}
    \end{tikzpicture}
    % 
	\caption{ Convergence test for the high-fidelity model, i.e. the classical TPS with finite elements.
	Left: Convergence of the error with respect to the mesh size;
	Right: Dependence of the minimum inf-sup constant of the TPS systems (over the time steps) on the mesh size.}
	\label{fig:conv_h_HF}
\end{figure}
